Forward LTLf Synthesis: DPLL At Work

This paper proposes a new AND-OR graph search framework for synthesis of Linear Temporal Logic on finite traces (\LTLf), that overcomes some limitations of previous approaches. Within such framework, we devise a procedure inspired by the Davis-Putnam-Logemann-Loveland (DPLL) algorithm to generate the next available agent-environment moves in a truly depth-first fashion, possibly avoiding exhaustive enumeration or costly compilations. We also propose a novel equivalence check for search nodes based on syntactic equivalence of state formulas. Since the resulting procedure is not guaranteed to terminate, we identify a stopping condition to abort execution and restart the search with state-equivalence checking based on Binary Decision Diagrams (BDD), which we show to be correct. The experimental results show that in many cases the proposed techniques outperform other state-of-the-art approaches. Our implementation Nike competed in the LTLf Realizability Track in the 2023 edition of SYNTCOMP, and won the competition.

==> notes.tex <==
R1:

The program corresponding to the hash-based state equivalence check function cannot guarantee termination. Although the stop condition is proposed in the paper to solve this problem, it is not proved that the stop condition can guarantee termination.

  solution: simple Theorem on termination

The paper is hard to follow. I think only experts in LTLf synthesis can understand the paper.

  ?

This paper contains too many dense symbols and notations without any explanations starting from Section Preliminaries. So this paper is less readable.

    solution: improve/expand preliminaries

How to apply the DPLL-like algorithm to extend search node in LTLf synthesis is not clearly stated in this paper. This is the main contribution of this paper. So I cannot determine if this is an incremental work or a significant improvement.

  solution: 
    1) add example, 
    2) improve formalization and proofs,
    3) reduce space to BDD check and Hash check

BDD-based and Hash-Consing-based state equivalence check was proposed, and is not novelty.

    solution: give it less importance (although hash-consing was not considered earlier in the literature!)
    show equivalences with literature


Section Preliminaries introduces the neXt Normal Form(XNF) of the LTLf formula and the Negation Normal Form (NNF) of the LTLf formula. What is the specific relationship between the two and the LTLf Formula Progression? Which form of LTLf formula is used in subsequent algorithms?

    highlight relationship
    specify use of formula


The core algorithm section as DPLL-based Forward Synthesis is a variant of DPLL algorithm, and DPLL is a complete algorithm based on backtracking algorithm and used to solve the proposition satisfiability problem in the conjunctive normal form (CNF). How does DPLL improve and apply to solve the problem of LTLf synthesis? What is the ideological logic behind it?

    explain ideological logic behind the algorithm

Figure 1(b) of Section Implementation and Experiments: The benchmark Single Counter (20), six combinations of Nike are all worse than Backward algorithm Lydia and the benchmark Nim (24), six combinations of Nike are all worse than Forward algorithm Cynthia. Could you provide a brief explanation of the above experimental results.

    explain experimental results

************************************
************************************


R2

On the other hand, the proposed procedure differs from (de Giacomo et al 2022) only in two respects that are more implementation aspects more than conceptual changes. Moreover, the modified equivalence check based on syntactic equivalence of formulae is rather simple, and as the authors write themselves, not really new.
The novelty thus seems limited.


    highlight novelties


Second, the presentation is not optimal.
- Important preliminaries are not explained, so that the presentation is in my opinion not self-contained.
-  did not grasp the problem with the previous procedure before consulting (de Giacomo et al 2022).
- Moreover, explanations are unclear and/or incomplete in several important points (see detailed comments below). 
- An example that shows how the two implementations differ would be extremely helpful. 

    IMPORTANT: add example



Here a procedure GetArcs is mentioned, but the new procedure in Algorithm 2 has a different name. The modification to Algorithm 1 does thus not become very clear.
It would be helpful to present the complete, modofoed algorithm (at least in the appendix).

    
